Predicting Parameter Change's Effect on Cellular Network Time Series

The cellular network provides convenient network access for ever-growing mobile phones. During the continuous optimization, operators can adjust cell parameters to enhance the Quality of Service (QoS) flexibly. A precise prediction of the parameter change's effect can help operators make proper parameter adjustments. This work focuses on predicting cell status (like the workload and QoS) after adjusting the cell parameters. The prediction will be conducted before an adjustment is actually applied to provide an early inspection. As it can be hard for available parameter adjustments with a limited number to cover all the parameter and user behavior combinations, we propose ParaSeer fusing domain knowledge on parameter adjustments into data-driven time series forecasting. ParaSeer organizes several pre-trained Transformers for adjustment-free time series forecasting, utilizing plenty of adjustment-free data. On the other hand, ParaSeer models the effect of adjusting the transmission power and cell individual offset (CIO) as a multiplier for the workload. We derive a formula to calculate the multiplier from the underlying mechanism of those two parameters, helping ParaSeer eliminate the thirst for data with parameter adjustments. We compare ParaSeer with baselines on two real-world datasets, where ParaSeer outperforms the best baseline by more than 25.8% in terms of RMSE. The extensive experiments further illustrate the contributions of ParaSeer's components.

==> img/cells-constant.tex <==
\pgfmathsetmacro{\SqrtThree}{sqrt(3)}
\pgfmathsetmacro{\ISD}{1.5} % inter site distance (in cm)
\pgfmathsetmacro{\BEL}{\ISD * \SqrtThree / 3} % border edge length
\pgfmathsetmacro{\THETA}{60}
\pgfmathsetmacro{\BETA}{0.5}
\pgfmathsetmacro{\GAMMA}{\THETA / 2 - asin(sqrt(\BETA) * sin(\THETA / 2))}
\pgfmathsetmacro{\CCSD}{\BETA / (1 - \BETA) * \ISD} % circle center-site distance
\pgfmathsetmacro{\RADIUS}{sqrt(\BETA) / (1 - \BETA) * \ISD}
\pgfmathsetmacro{\CBSD}{\RADIUS - \CCSD} % circle border-site distance

\coordinate (site-0) at (0cm, 0cm);
\coordinate (site-1) at (\ISD cm * \SqrtThree / 2, \ISD * 0.5cm);
\coordinate (site-2) at (0cm, \ISD cm);
\coordinate (site-3) at (-\ISD cm * \SqrtThree / 2, \ISD * 0.5cm);
\coordinate (site-4) at (-\ISD cm * \SqrtThree / 2, -\ISD * 0.5cm);
\coordinate (site-5) at (0cm, -\ISD cm);
\coordinate (site-6) at (\ISD cm * \SqrtThree / 2, -\ISD * 0.5 cm);

\coordinate (vertex-1) at (\BEL cm, 0cm);
\coordinate (vertex-1-1) at (\BEL cm * 1.5, 0cm);
\coordinate (vertex-2) at (\BEL * 0.5cm, \BEL cm * \SqrtThree / 2);
\coordinate (vertex-2-2) at (\BEL cm * 0.75, \BEL cm * \SqrtThree * 0.75);
\coordinate (vertex-3) at (-\BEL * 0.5cm, \BEL cm * \SqrtThree / 2);
\coordinate (vertex-3-3) at (-\BEL cm * 0.75, \BEL cm * \SqrtThree * 0.75);
\coordinate (vertex-4) at (-\BEL cm, 0cm);
\coordinate (vertex-4-4) at (-\BEL cm * 1.5, 0cm);
\coordinate (vertex-5) at (-\BEL * 0.5cm, -\BEL cm * \SqrtThree / 2);
\coordinate (vertex-5-5) at (-\BEL cm * 0.75, -\BEL cm * \SqrtThree * 0.75);
\coordinate (vertex-6) at (\BEL * 0.5cm, -\BEL cm * \SqrtThree / 2);
\coordinate (vertex-6-6) at (\BEL cm * 0.75, -\BEL cm * \SqrtThree * 0.75);

